Duality and Stability in Complex Multiagent State-Dependent Network Dynamics

Despite significant progress on stability analysis of conventional multiagent networked systems with weakly coupled state-network dynamics, most of the existing results have shortcomings in addressing multiagent systems with highly coupled state-network dynamics. Motivated by numerous applications of such dynamics, in our previous work [1], we initiated a new direction for stability analysis of such systems that uses a sequential optimization framework. Building upon that, in this paper, we extend our results by providing another angle on multiagent network dynamics from a duality perspective, which allows us to view the network structure as dual variables of a constrained nonlinear program. Leveraging that idea, we show that the evolution of the coupled state-network multiagent dynamics can be viewed as iterates of a primal-dual algorithm for a static constrained optimization/saddle-point problem. This view bridges the Lyapunov stability of state-dependent network dynamics and frequently used optimization techniques such as block coordinated descent, mirror descent, the Newton method, and the subgradient method. As a result, we develop a systematic framework for analyzing the Lyapunov stability of state-dependent network dynamics using techniques from nonlinear optimization. Finally, we support our theoretical results through numerical simulations from social science.

==> thesisrefs.tex <==
@STRING{IEEE_J_EC         = "{IEEE} Trans. En. Conv."}
@STRING{IEEE_J_PWRE       = "{IEEE} Trans. Power Electron."}
@STRING{IEEE_J_PWRS       = "{IEEE} Trans. Power Syst."}
@STRING{IEEE_J_MAG        = "{IEEE} Trans. Magn."}
@STRING{J_NUM_ENG         = "Int. J. Numer. Meth. Engng."}
@STRING{ENG_ANAL          = "Eng. Anal."}
@STRING{IEEE_J_EDU        = "{IEEE} Trans. Educ."}
@STRING{IEEE_J_MTT        = "{IEEE} Trans. Microwave Theory Tech."}
@STRING{IEEE_J_IA         = "{IEEE} Trans. Ind. Applicat."}
@STRING{IEEE_J_AntProp    = "{IEEE} Trans. Ant. and Prop."}







@inproceedings{balcan2015commitment,
  title={Commitment without regrets: {O}nline learning in stackelberg security games},
  author={Balcan, Maria-Florina and Blum, Avrim and Haghtalab, Nika and Procaccia, Ariel D},
  booktitle={Proceedings of the Sixteenth ACM Conference on Economics and Computation},
  pages={61-78},
  year={2015},
  organization={ACM}
}


@inproceedings{letchford2009learning,
  title={Learning and approximating the optimal strategy to commit to},
  author={Letchford, Joshua and Conitzer, Vincent and Munagala, Kamesh},
  booktitle={International Symposium on Algorithmic Game Theory},
  pages={250--262},
  year={2009},
  organization={Springer}
}

@inproceedings{blum2014learning,
  title={Learning optimal commitment to overcome insecurity},
  author={Blum, Avrim and Haghtalab, Nika and Procaccia, Ariel D},
  booktitle={Advances in Neural Information Processing Systems},
  pages={1826--1834},
  year={2014}
}

@inproceedings{marecki2012playing,
  title={Playing repeated {S}tackelberg games with unknown opponents},
  author={Marecki, Janusz and Tesauro, Gerry and Segal, Richard},
  booktitle={Proceedings of the 11th International Conference on Autonomous Agents and Multiagent Systems-Volume 2},
  pages={821--828},
  year={2012},
  organization={International Foundation for Autonomous Agents and Multiagent Systems}
}

@inproceedings{xu2016playing,
  title={Playing Repeated Security Games with No Prior Knowledge},
  author={Xu, Haifeng and Tran-Thanh, Long and Jennings, Nicholas R},
  booktitle={Proceedings of the 2016 International Conference on Autonomous Agents \& Multiagent Systems},
  pages={104--112},
  year={2016},
  organization={International Foundation for Autonomous Agents and Multiagent Systems}
}

@article{yan2014integrated,
  title={Integrated security analysis on cascading failure in complex networks},
  author={Yan, Jun and He, Haibo and Sun, Yan},
  journal={IEEE Transactions on Information Forensics and Security},
  volume={9},
  number={3},
  pages={451--463},
  year={2014},
  publisher={IEEE}
}

@article{etesami2016complexity,
  title={Complexity of equilibrium in competitive diffusion games on social networks},
  author={Etesami, S. Rasoul and Ba\c{s}ar, Tamer},
  journal={Automatica},
  volume={68},
  pages={100--110},
  year={2016},
  publisher={Elsevier}
}

@inproceedings{grossklags2008secure,
  title={Secure or insure?: {A} game-theoretic analysis of information security games},
  author={Grossklags, Jens and Christin, Nicolas and Chuang, John},
  booktitle={Proceedings of the 17th international Conference on World Wide Web},
  pages={209--218},
  year={2008},
  organization={ACM}
}

@article{laszka2015survey,
  title={A survey of interdependent information security games},
  author={Laszka, Aron and Felegyhazi, Mark and Buttyan, Levente},
  journal={ACM Computing Surveys (CSUR)},
  volume={47},
  number={2},
  pages={23},
  year={2015},
  publisher={ACM}
}

@article{kaivanto2014effect,
  title={The Effect of Decentralized Behavioral Decision Making on System-Level Risk},
  author={Kaivanto, Kim},
  journal={Risk Analysis},
  volume={34},
  number={12},
  pages={2121--2142},
  year={2014},
  publisher={Wiley Online Library}
}

@inproceedings{casey2014cyber,
  title={Cyber security via signaling games: Toward a science of cyber security},
  author={Casey, William and Morales, Jose A and Nguyen, Thomson and Spring, Jonathan and Weaver, Rhiannon and Wright, Evan and Metcalf, Leigh and Mishra, Bud},
  booktitle={International Conference on Distributed Computing and Internet Technology},
  pages={34--42},
  year={2014},
  organization={Springer}
}

@techreport{gibson2013applied,
  title={Applied Hypergame Theory for Network Defense},
  author={Gibson, Alan S},
  year={2013},
  institution={DTIC Document}
}

@inproceedings{house2010hypergame,
  title={Hypergame theory applied to cyber attack and defense},
  author={House, James Thomas and Cybenko, George},
  booktitle={SPIE Defense, Security, and Sensing},
  pages={766604--766604},
  year={2010},
  organization={International Society for Optics and Photonics}
}

@article{pawlick2015deception,
  title={Deception by design: evidence-based signaling games for network defense},
  author={Pawlick, Jeffrey and Zhu, Quanyan},
  journal={arXiv preprint arXiv:1503.05458},
  year={2015}
}

@article{khanafer2016robust,
  title={Robust distributed averaging: When are potential-theoretic strategies optimal?},
  author={Khanafer, Ali and Ba\c{s}ar, Tamer},
  journal={IEEE Transactions on Automatic Control},
  volume={61},
  number={7},
  pages={1767-1779},
  year={2016},
  publisher={IEEE}
}

@article{etesami2015game,
  title={Game-theoretic analysis of the {H}egselmann-{K}rause model for opinion dynamics in finite dimensions},
  author={Etesami, Seyed Rasoul and Ba\c{s}ar, Tamer},
  journal={IEEE Transactions on Automatic Control},
  volume={60},
  number={7},
  pages={1886--1897},
  year={2015},
  publisher={IEEE}
}


@article{jadbabaie2003coordination,
  title={Coordination of groups of mobile autonomous agents using nearest neighbor rules},
  author={Jadbabaie, Ali and Lin, Jie and Morse, A Stephen},
  journal={IEEE Transactions on automatic control},
  volume={48},
  number={6},
  pages={988-1001},
  year={2003},
  publisher={IEEE}
}

@article{etesami2016convergence,
  title={Convergence time for unbiased quantized consensus over static and dynamic networks},
  author={Etesami, Seyed Rasoul and Ba\c{s}ar, Tamer},
  journal={IEEE Transactions on Automatic Control},
  volume={61},
  number={2},
  pages={443-455},
  year={2016},
  publisher={IEEE}
}

@article{bacsar2016convergence,
  title={Convergence time of quantized {M}etropolis consensus over time-varying networks},
  author={Ba{\c{s}}ar, Tamer and Etesami, Seyed Rasoul and Olshevsky, Alex},
  journal={IEEE Transactions on Automatic Control},
  volume={61},
  number={12},
  pages={4048-4054},
  year={2016},
  publisher={IEEE}
}

@article{immorlica2011dueling,
	Author = {Immorlica, Nicole and Kalai, Adam Tauman and Lucier, Brendan and Moitra, Ankur and Postlewaite, Andrew and Tennenholtz, Moshe},
	Booktitle = {Proc. the 43rd Annual ACM Symposium on Theory of Computing},
	Date-Added = {2016-10-18 20:41:10 +0000},
	Date-Modified = {2016-10-18 20:44:20 +0000},
	Pages = {215--224},
	Title = {Dueling algorithms},
	Year = {2011}}

@inproceedings{kiekintveld2009computing,
	Author = {Kiekintveld, Christopher and Jain, Manish and Tsai, Jason and Pita, James and Ord{\'o}{\~n}ez, Fernando and Tambe, Milind},
	Booktitle = {Proceedings of The 8th International Conference on Autonomous Agents and Multiagent Systems-Volume 1},
	Organization = {International Foundation for Autonomous Agents and Multiagent Systems},
	Pages = {689--696},
	Title = {Computing optimal randomized resource allocations for massive security games},
	Year = {2009}}

@book{tambe2011security,
	Author = {Tambe, M.},
	Publisher = {Cambridge University Press},
	Title = {Security and game theory: Algorithms, deployed systems, lessons learned},
	Year = {2011}}

@article{buldyrev2010catastrophic,
	Author = {Buldyrev, Sergey V and Parshani, Roni and Paul, Gerald and Stanley, H Eugene and Havlin, Shlomo},
	Journal = {Nature},
	Number = {7291},
	Pages = {1025--1028},
	Publisher = {Nature Publishing Group},
	Title = {Catastrophic cascade of failures in interdependent networks},
	Volume = {464},
	Year = {2010}}

@incollection{gueye2012towards,
	Author = {Gueye, A. and Marbukh, V. and Walrand, J. C.},
	Booktitle = {Game Theory for Networks},
	Pages = {259--274},
	Publisher = {Springer},
	Title = {Towards a Metric for Communication Network Vulnerability to Attacks: A Game Theoretic Approach},
	Year = {2012}}

@article{washburn1995two,
	Author = {Washburn, A. and Wood, K.},
	Journal = {Operations Research},
	Number = {2},
	Pages = {243--251},
	Publisher = {INFORMS},
	Title = {Two-person zero-sum games for network interdiction},
	Volume = {43},
	Year = {1995}}

@inproceedings{yen2015sparse,
	Author = {Yen, I. E. and Zhong, K. and Hsieh, C. and Ravikumar, P. K. and Dhillon, I. S.},
	Booktitle = {Advances in Neural Information Processing Systems (NIPS)},
	Pages = {2359--2367},
	Title = {Sparse linear programming via primal and dual augmented coordinate descent},
	Year = {2015}}

@article{kennes2013computational,
	Author = {Kennes, R. and Smets, P.},
	Journal = {arXiv preprint arXiv:1304.1122},
	Title = {Computational aspects of the Mobius transform},
	Year = {2013}}

@book{motwani2010randomized,
	Author = {Motwani, Rajeev and Raghavan, Prabhakar},
	Publisher = {Chapman \& Hall/CRC},
	Title = {Randomized algorithms},
	Year = {2010}}
	
@book{von1934marktform,
  title={Marktform und gleichgewicht},
  author={Von Stackelberg, Heinrich},
  year={1934},
  publisher={J. springer}
}

@article{harsanyi2004games,
  title={Games with incomplete information played by “Bayesian” players, i–iii: part i. the basic model},
  author={Harsanyi, John C},
  journal={Management science},
  volume={50},
  number={12\_supplement},
  pages={1804--1817},
  year={2004},
  publisher={INFORMS}
}

@inproceedings{wang2017security,
  title={Security Game with Non-additive Utilities and Multiple Attacker Resources},
  author={Wang, Sinong and Shroff, Ness},
  booktitle={Proceedings of the 2017 ACM SIGMETRICS/International Conference on Measurement and Modeling of Computer Systems},
  pages={10--10},
  year={2017},
  organization={ACM}
}

@article{wang2016non,
  title={Non-additive Security Game},
  author={Wang, Sinong and Liu, Fang and Shroff, Ness},
  journal={AAAI 17},
  year={2017}
}

@inproceedings{letchford2013solving,
  title={Solving Security Games on Graphs via Marginal Probabilities.},
  author={Letchford, Joshua and Conitzer, Vincent},
  booktitle={AAAI},
  year={2013}
}

@inproceedings{paruchuri2008playing,
  title={Playing games for security: An efficient exact algorithm for solving Bayesian Stackelberg games},
  author={Paruchuri, Praveen and Pearce, Jonathan P and Marecki, Janusz and Tambe, Milind and Ordonez, Fernando and Kraus, Sarit},
  booktitle={Proceedings of the 7th international joint conference on Autonomous agents and multiagent systems-Volume 2},
  pages={895--902},
  year={2008},
  organization={International Foundation for Autonomous Agents and Multiagent Systems}
}

@article{von2004leadership,
  title={Leadership with commitment to mixed strategies},
  author={Von Stengel, Bernhard and Zamir, Shmuel},
  year={2004},
  publisher={Centre for Discrete and Applicable Mathematics, London School of Economics and Political Science}
}

@article{tsai2009iris,
  title={IRIS-A Tool for Strategic Security Allocation in Transportation Networks},
  author={Tsai, Jason and Rathi, Shyamsunder and Kiekintveld, Christopher and Ord{\'o}{\~n}ez, Fernando and Tambe, Milind},
  year={2009}
}

@inproceedings{korzhyk2011security,
  title={Security games with multiple attacker resources},
  author={Korzhyk, Dmytro and Conitzer, Vincent and Parr, Ronald},
  booktitle={IJCAI Proceedings-International Joint Conference on Artificial Intelligence},
  volume={22},
  number={1},
  pages={273--279},
  year={2011},
  organization={Citeseer}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%














@article{MOJ-SN:15,
  author =        {M. O. Jackson and S. Nei},
  journal =       {Proceedings of the National Academy of Sciences},
  number =        {50},
  pages =         {15277-15284},
  title =         {Networks of military alliances, wars, and
                   international trade},
  volume =        {112},
  year =          {2015},
  abstract =      {We investigate the role of networks of alliances in
                   preventing (multilateral) interstate wars. We first
                   show that, in the absence of international trade, no
                   network of alliances is peaceful and stable. We then
                   show that international trade induces peaceful and
                   stable networks: Trade increases the density of
                   alliances so that countries are less vulnerable to
                   attack and also reduces countries’ incentives to
                   attack an ally. We present historical data on wars
                   and trade showing that the dramatic drop in
                   interstate wars since 1950 is paralleled by a
                   densification and stabilization of trading
                   relationships and alliances. Based on the model we
                   also examine some specific relationships, finding
                   that countries with high levels of trade with their
                   allies are less likely to be involved in wars with
                   any other countries (including allies and nonallies),
                   and that an increase in trade between two countries
                   correlates with a lower chance that they will go to
                   war with each other.},
  doi =           {10.1073/pnas.1520970112},
}

@article{RA-WM-RET-DSB-EB:95,
  author =        {R. Axelrod and W. Mitchell and R. E. Thomas and
                   D. S. Bennett and E. Bruderer},
  journal =       {Management Science},
  pages =         {1493--1508},
  title =         {Coalition Formation in Standard-Setting Alliances},
  volume =        {41},
  year =          {1995},
  doi =           {10.1287/mnsc.41.9.1493},
}

@article{BS-RP:00,
  author =        {B. Skyrms and R. Pemantle},
  journal =       {Proceedings of the National Academy of Sciences},
  number =        {16},
  pages =         {9340-9346},
  title =         {A Dynamic Model of Social Network Formation},
  volume =        {97},
  year =          {2000},
  doi =           {10.1073/pnas.97.16.9340},
}

@incollection{MOJ:05,
  author =        {M. O. Jackson},
  booktitle =     {Group Formation in Economics; Networks, Clubs and
                   Coalitions},
  editor =        {Demange, G. and Wooders, M.},
  publisher =     {Cambridge University Press},
  title =         {A Survey of Models of Network Formation: Stability
                   and Efficiency},
  year =          {2005},
  url =           {https://web.stanford.edu/~jacksonm/netsurv.pdf},
}

@article{AvdR:11,
  author =        {A. {van~de~Rijt}},
  journal =       {Journal of Mathematical Sociology},
  number =        {1-3},
  pages =         {94-113},
  title =         {The Micro-Macro Link for the Theory of Structural
                   Balance},
  volume =        {35},
  year =          {2011},
  doi =           {10.1080/0022250X.2010.532262},
}

@article{SS-KRA:13,
  author =        {S. Simon and K. R. Apt},
  journal =       {Journal of Logic and Computation},
  pages =         {1--36},
  title =         {Social Network Games},
  volume =        {25},
  year =          {2013},
  doi =           {10.1093/logcom/ext012},
}

@book{WHS:10,
  author =        {W. H. Sandholm},
  publisher =     {MIT Press},
  title =         {Population Games and Evolutionary Dynamics},
  year =          {2010},
  isbn =          {0262195879},
}

@article{FH:46,
  author =        {F. Heider},
  journal =       {The Journal of Psychology},
  number =        {1},
  pages =         {107--112},
  title =         {Attitudes and Cognitive Organization},
  volume =        {21},
  year =          {1946},
  doi =           {10.1080/00223980.1946.9917275},
}

@article{DC-FH:56,
  author =        {D. Cartwright and F. Harary},
  journal =       {Psychological Review},
  number =        {5},
  pages =         {277},
  title =         {Structural balance: a generalization of {H}eider's
                   theory},
  volume =        {63},
  year =          {1956},
  doi =           {10.1037/h0046049},
}

@book{NEF:98,
  author =        {N. E. Friedkin},
  publisher =     {Cambridge University Press},
  series =        {Structural Analysis in the Social Sciences},
  title =         {A Structural Theory of Social Influence},
  year =          {1998},
  isbn =          {9780521454827},
}

@article{TA-PLK-SR:05,
  author =        {T. Antal and P. L. Krapivsky and S. Redner},
  journal =       {Physical Review E},
  number =        {3},
  pages =         {036121},
  title =         {Dynamics of social balance on networks},
  volume =        {72},
  year =          {2005},
  doi =           {10.1103/PhysRevE.72.036121},
}

@article{SAM-JK-RDK-SHS:11,
  author =        {S. A. Marvel and J. Kleinberg and R. D. Kleinberg and
                   S. H. Strogatz},
  journal =       {Proceedings of the National Academy of Sciences},
  number =        {5},
  pages =         {1771--1776},
  title =         {Continuous-time model of structural balance},
  volume =        {108},
  year =          {2011},
  doi =           {10.1073/pnas.1013213108},
}

@article{VAT-PVD-PDL:13,
  author =        {V. A. Traag and P. Van~Dooren and P. De~Leenheer},
  journal =       {PLOS ONE},
  number =        {4},
  pages =         {e60063},
  title =         {Dynamical Models Explaining Social Balance and
                   Evolution of Cooperation},
  volume =        {8},
  year =          {2013},
  doi =           {10.1371/journal.pone.0060063},
}

@article{XZ-DZ-FYW:15,
  author =        {X. Zheng and D. Zeng and F.-Y. Wang},
  journal =       {Information Systems Frontiers},
  number =        {5},
  pages =         {1077--1095},
  title =         {Social balance in signed networks},
  volume =        {17},
  year =          {2015},
  doi =           {10.1007/s10796-014-9483-8},
}

@article{PJ-NEF-FB:13n,
  author =        {P. Jia and N. E. Friedkin and F. Bullo},
  journal =       {IEEE Transactions on Network Science and Engineering},
  number =        {4},
  pages =         {286-298},
  title =         {The Coevolution of Appraisal and Influence Networks
                   leads to Structural Balance},
  volume =        {3},
  year =          {2016},
  abstract =      {In sociology, an appraisal structure, represented by
                   a signed matrix or a signed network, describes an
                   evaluative cognitive configuration among individuals.
                   In this article we argue that interpersonal
                   influences originate from positive interpersonal
                   appraisals and, in turn, adjust individuals'
                   appraisals of others. This mechanism amounts to a
                   coevolution process of interpersonal appraisals and
                   influences. We provide a mathematical formulation of
                   the coevolutionary dynamics, characterize the
                   invariant appraisal structures, and establish the
                   convergence properties for all possible initial
                   appraisals. Moreover, we characterize the
                   implications of our model to the study of signed
                   social networks. Specifically, our model predicts the
                   convergence of the interpersonal appraisal network to
                   a structure composed of multiple factions with
                   multiple followers. A faction is a group of
                   individuals with positive-complete interpersonal
                   appraisals among them. We discuss how this
                   factions-with-followers is a balanced structure with
                   respect to an appropriate generalized model of
                   balance theory.},
  doi =           {10.1109/TNSE.2016.2600058},
}

@article{WM-PCV-NEF-FB:17f,
  author =        {W. Mei and P. Cisneros-Velarde and N. E. Friedkin and
                   F. Bullo},
  journal =       {Automatica},
  month =         sep,
  note =          {Working Paper},
  title =         {Dynamic Social Balance and Convergent Appraisals via
                   Homophily and Influence Mechanisms},
  year =          {2017},
}

@inproceedings{MM-MF-PJK-HRR-MAS:11,
  address =       {San Diego, USA},
  author =        {M. Malekzadeh and M. Fazli and
                   P. {Jalaly~Khalidabadi} and H. R. Rabiee and
                   M. A. Safari},
  booktitle =     {Proceedings of 5th KDD workshop on Social Network
                   Analysis (SNA-KDD)},
  month =         aug,
  title =         {Social Balance and Signed Network Formation Games},
  year =          {2011},
}

@article{TH:16,
  author =        {T. Hiller},
  journal =       {Theoretical Economics},
  note =          {To appear},
  title =         {Friends and enemies: a model of signed network
                   formation},
  year =          {2016},
  abstract =      {I propose a simple model of signed network formation,
                   where agents make friends to extract payoffs from
                   weaker enemies. The model thereby accounts for the
                   interplay between friendship and alliance on one hand
                   and enmity and antagonism on the other. Nash
                   equilibrium configurations are such that, either
                   everyone is friends with everyone, or agents can be
                   partitioned into different sets, where agents within
                   the same set are friends and agents in different sets
                   are enemies. Any strong Nash equilibrium must be such
                   that a single agent is in an antagonistic
                   relationship with everyone else. Furthermore, we show
                   that Nash equilibria cannot be Pareto ranked. This
                   paper offers a game-theoretic foundation for a large
                   body of work on signed networks, called structural
                   balance theory, which has been studied in sociology,
                   social psychology, bullying, international relations
                   and applied physics. The paper also contributes to
                   the literature on contests and economics of
                   conflict.},
  url =           {http://EconPapers.repec.org/RePEc:the:publsh:1937},
}

@article{MH:02,
  author =        {Michael Howard},
  journal =       {Foreign Affairs},
  number =        {1},
  pages =         {8-13},
  publisher =     {Council on Foreign Relations},
  title =         {What's in a Name? {H}ow to Fight Terrorism},
  volume =        {81},
  year =          {2002},
  abstract =      {By declaring "war" on terrorism, the United States
                   has committed itself to decisive victory against an
                   intractable enemy and to a long march through "rogue"
                   states.},
  doi =           {10.2307/20032999},
}

@article{VEK:02,
  author =        {V. E. Krebs},
  journal =       {Connections},
  number =        {3},
  pages =         {43--52},
  title =         {Mapping networks of terrorist cells},
  volume =        {24},
  year =          {2002},
  url =           {https://insna.org/PDF/Connections/v24/2001_I-3-7.pdf},
}

@article{AP-AP:11,
  author =        {A. Perliger and A. Pedahzur},
  journal =       {PS: Political Science \& Politics},
  number =        {1},
  pages =         {45–50},
  title =         {Social Network Analysis in the Study of Terrorism and
                   Political Violence},
  volume =        {44},
  year =          {2011},
  doi =           {10.1017/S1049096510001848},
}

@book{SEF:12,
  author =        {S. F. Everton},
  publisher =     {Cambridge University Press},
  title =         {Disrupting Dark Networks},
  year =          {2012},
}

@misc{PVF-RW:17,
  author =        {P. Vos~Fellman and R. Wright},
  note =          {arXiv preprint},
  title =         {Modeling Terrorist Networks, {C}omplex Systems at the
                   Mid-range},
  year =          {2017},
  url =           {https://arxiv.org/abs/1706.08602},
}

@article{HWH:00,
  author =        {H. W. Hethcote},
  journal =       {SIAM Review},
  number =        {4},
  pages =         {599--653},
  title =         {The Mathematics of Infectious Diseases},
  volume =        {42},
  year =          {2000},
  doi =           {10.1137/S0036144500371907},
}

@article{RPS-CC-PVM-AV:15,
  author =        {R. Pastor-Satorras and C. Castellano and
                   P. Van~Mieghem and A. Vespignani},
  journal =       {Reviews of Modern Physics},
  pages =         {925--979},
  title =         {Epidemic processes in complex networks},
  volume =        {87},
  year =          {2015},
  doi =           {10.1103/RevModPhys.87.925},
}

@article{CN-VMP-GJP:16,
  author =        {C. Nowzari and V. M. Preciado and G. J. Pappas},
  journal =       {{IEEE} Control Systems},
  number =        {1},
  pages =         {26-46},
  title =         {Analysis and Control of Epidemics: {A} Survey of
                   Spreading Processes on Complex Networks},
  volume =        {36},
  year =          {2016},
  doi =           {10.1109/MCS.2015.2495000},
}

@article{WM-SM-SZ-FB:16f,
  author =        {W. Mei and S. Mohagheghi and S. Zampieri and
                   F. Bullo},
  journal =       {Annual Reviews in Control},
  month =         jan,
  note =          {To appear},
  title =         {On the Dynamics of Deterministic Epidemic Propagation
                   over Networks},
  year =          {2017},
  abstract =      {In this work we review a class of deterministic
                   nonlinear models for the propagation of infectious
                   diseases over contact networks with
                   strongly-connected topologies. We consider network
                   models for susceptible-infected (SI),
                   susceptible-infected-susceptible (SIS), and
                   susceptible-infected-recovered (SIR) settings. In
                   each setting, we provide a comprehensive nonlinear
                   analysis of equilibria, stability properties,
                   convergence, monotonicity, positivity, and threshold
                   conditions. For the network SI setting, specific
                   contributions include establishing its equilibria,
                   stability, and positivity properties. For the network
                   SIS setting, we review a well- known deterministic
                   model, provide novel results on the computation and
                   characterization of the endemic state (when the
                   system is above the epidemic threshold), and present
                   alternative proofs for some of its properties.
                   Finally, for the network SIR setting, we propose
                   novel results for transient behavior, threshold
                   conditions, stability properties, and asymptotic
                   convergence. These results are analogous to those
                   well-known for the scalar case. In addition, we
                   provide a novel iterative algorithm to compute the
                   asymptotic state of the network SIR system.},
}

@article{CC-SF-VL:09,
  author =        {Castellano, C. and Fortunato, S. and Loreto, V.},
  journal =       {Reviews of Modern Physics},
  number =        {2},
  pages =         {591--646},
  title =         {Statistical Physics of Social Dynamics},
  volume =        {81},
  year =          {2009},
  doi =           {10.1103/RevModPhys.81.591},
}


@book{friedkin2011social,
  title={Social influence network theory: {A} sociological examination of small group dynamics},
  author={Friedkin, Noah E and Johnsen, Eugene C},
  volume={33},
  year={2011},
  publisher={Cambridge University Press}
}

@article{AVP-RT:17,
  author =        {A. V. Proskurnikov and R. Tempo},
  journal =       {Annual Reviews in Control},
  pages =         {65-79},
  title =         {A Tutorial on Modeling and Analysis of Dynamic Social
                   Networks. {Part I}},
  volume =        {43},
  year =          {2017}
}

@article{PJ-AM-NEF-FB:13d,
  author =        {P. Jia and A. MirTabatabaei and N. E. Friedkin and
                   F. Bullo},
  journal =       {SIAM Review},
  number =        {3},
  pages =         {367-397},
  title =         {Opinion Dynamics and The Evolution of Social Power in
                   Influence Networks},
  volume =        {57},
  year =          {2015},
  abstract =      {This paper studies the evolution of self appraisal,
                   social power and interpersonal influences for a group
                   of individuals who discuss and form opinions about a
                   sequence of issues. Our empirical model combines the
                   averaging rule by DeGroot to describe opinion
                   formation processes and the reflected appraisal
                   mechanism by Friedkin to describe the dynamics of
                   individuals' self appraisal and social power. Given a
                   set of relative interpersonal weights, the
                   DeGroot-Friedkin model predicts the evolution of the
                   influence network governing the opinion formation
                   process. We provide a rigorous mathematical
                   formulation of the influence network dynamics,
                   characterize its equilibria and establish its
                   convergence properties for all possible structures of
                   the relative interpersonal weights and corresponding
                   eigenvector centrality scores. The model predicts
                   that the social power ranking among individuals is
                   asymptotically equal to their centrality ranking,
                   that social power tends to accumulate at the top of
                   the hierarchy, and that an autocratic (resp.
                   democratic) power structure arises when the
                   centrality scores are maximally non-uniform (resp.
                   uniform).},
  doi =           {10.1137/130913250},
}

@article{NEF-FB:16d,
  author =        {N. E. Friedkin and F. Bullo},
  journal =       {Proceedings of the National Academy of Sciences},
  note =          {To appear},
  title =         {How Truth Wins in Opinion Dynamics along Issue
                   Sequences},
  year =          {2017},
  abstract =      {How truth wins in social groups is an important open
                   problem. Classic experiments on social groups dealing
                   with truth statement issues present mixed findings on
                   the conditions of truth abandonment and reaching a
                   consensus on the truth. No theory has been developed
                   and evaluated that might integrate these findings
                   with a mathematical model of the interpersonal
                   influence system that alters some or all of its
                   members' positions on an issue. In this article, we
                   provide the first evidence that a general model in
                   the network science on opinion dynamics substantially
                   clarifies how truth wins in groups. the hazard rate
                   of adopting false positions on truth statements is
                   substantial and that truth propagation is not a viral
                   contagion in which a true position is automatically
                   adopted by anyone who comes into contact with it.},
}

@article{NEF-AVP-RT-SEP:16,
  author =        {N. E. Friedkin and A. V. Proskurnikov and R. Tempo and
                   S. E. Parsegov},
  journal =       {Science},
  number =        {6310},
  pages =         {321--326},
  title =         {Network science on belief system dynamics under logic
                   constraints},
  volume =        {354},
  year =          {2016},
  abstract =      {People tend to structure their beliefs in a way that
                   appears consistent to them. But how do some beliefs
                   within groups persist in the face of social pressure,
                   whereas others change and, by changing, influence a
                   cascade of other beliefs? Friedkin et al. developed a
                   model that can describe complexes of attitudes in a
                   group that interact and change (see the Perspective
                   by Butts). Their model revealed how the changing
                   views of the U.S. population on the existence of
                   weapons of mass destruction in Iraq changed their
                   views on whether the invasion by the United States
                   was justified. Breakthroughs have been made in
                   algorithmic approaches to understanding how
                   individuals in a group influence each other to reach
                   a consensus. However, what happens to the group
                   consensus if it depends on several statements, one of
                   which is proven false? Here, we show how the
                   existence of logical constraints on beliefs affect
                   the collective convergence to a shared belief system
                   and, in contrast, how an idiosyncratic set of
                   arbitrarily linked beliefs held by a few may become
                   held by many.},
  doi =           {10.1126/science.aag2624},
}

@article{CA:13,
  author =        {C. Altafini},
  journal =       {IEEE Transactions on Automatic Control},
  number =        {4},
  pages =         {935--946},
  title =         {Consensus problems on networks with antagonistic
                   interactions},
  volume =        {58},
  year =          {2013},
  doi =           {10.1109/TAC.2012.2224251},
}

@inproceedings{JMH:14,
  author =        {J. M. Hendrickx},
  booktitle =     {{IEEE} Conf.\ on Decision and Control},
  month =         dec,
  pages =         {2118-2123},
  title =         {A lifting approach to models of opinion dynamics with
                   antagonisms},
  year =          {2014},
  doi =           {10.1109/CDC.2014.7039711},
}

@article{WX-MC-KHJ:16,
  author =        {W. Xia and M. Cao and K. H. Johansson},
  journal =       {IEEE Transactions on Control of Network Systems},
  number =        {1},
  pages =         {46-56},
  title =         {Structural Balance and Opinion Separation in
                   Trust-Mistrust Social Networks},
  volume =        {3},
  year =          {2016},
  doi =           {10.1109/TCNS.2015.2437528},
}

@article{WM-NEF-KL-FB:16g,
  author =        {W. Mei and N. E. Friedkin and K. Lewis and F. Bullo},
  journal =       {IEEE Transactions on Automatic Control},
  month =         sep,
  note =          {Submitted},
  title =         {Dynamic Models of Appraisal Networks Explaining
                   Collective Learning},
  year =          {2016},
  abstract =      {This paper proposes models of learning process in
                   teams of individuals who collectively execute a
                   sequence of tasks and whose actions are determined by
                   individual skill levels and networks of interpersonal
                   appraisals and influence. The closely-related
                   proposed models have increasing complexity, starting
                   with a centralized manager-based assignment and
                   learning model, and finishing with a social model of
                   interpersonal appraisal, assignments, learning, and
                   influences. We show how rational optimal behavior
                   arises along the task sequence for each model, and
                   discuss conditions of suboptimality. Our models are
                   grounded in replicator dynamics from evolutionary
                   games, influence networks from mathematical
                   sociology, and transactive memory systems from
                   organization science.},
}

@article{YN-VYP:13,
  author =        {Y. Nesterov and V. Y. Protasov},
  journal =       {SIAM Journal on Matrix Analysis and Applications},
  number =        {3},
  pages =         {999--1013},
  title =         {Optimizing the Spectral Radius},
  volume =        {34},
  year =          {2013},
  doi =           {10.1137/110850967},
}

@inproceedings{AG-SB:06,
  author =        {A. Ghosh and S. Boyd},
  booktitle =     {{IEEE} Conf.\ on Decision and Control},
  month =         dec,
  pages =         {6605-6611},
  title =         {Growing Well-connected Graphs},
  year =          {2006},
  doi =           {10.1109/CDC.2006.377282},
}

@article{AG-SB-AS:08,
  author =        {A. Ghosh and S. Boyd and A. Saberi},
  journal =       {SIAM Review},
  number =        {1},
  pages =         {37--66},
  title =         {Minimizing effective resistance of a graph},
  volume =        {50},
  year =          {2008},
  doi =           {10.1137/050645452},
}

@article{SB-PD-LX:04,
  author =        {S. Boyd and P. Diaconis and L. Xiao},
  journal =       {SIAM Review},
  number =        {4},
  pages =         {667--689},
  title =         {Fastest mixing {M}arkov chain on a graph},
  volume =        {46},
  year =          {2004},
  doi =           {10.1137/S0036144503423264},
}

@article{RP-PA-FB:14b,
  author =        {R. Patel and P. Agharkar and F. Bullo},
  journal =       {IEEE Transactions on Automatic Control},
  number =        {12},
  pages =         {3156-3157},
  title =         {Robotic Surveillance and {M}arkov Chains with Minimal
                   Weighted {K}emeny Constant},
  volume =        {60},
  year =          {2015},
  abstract =      {This article provides analysis and optimization
                   results for the \emph{mean first passage time}, also
                   known as the \emph{Kemeny constant}, of a Markov
                   chain. First, we generalize the notion of Kemeny
                   constant to environments with heterogeneous travel
                   and service times, denote this generalization as the
                   \emph{weighted Kemeny constant}, and we characterize
                   its properties. Second, for reversible Markov chains,
                   we show that the minimization of the Kemeny constant
                   and its weighted counterpart can be formulated as
                   convex optimization problems and, moreover, as
                   semidefinite programs. Third, we apply these results
                   to the design of stochastic surveillance strategies
                   for quickest detection of anomalies in network
                   environments. We numerically illustrate the proposed
                   design: compared with other well-known Markov chains,
                   the performance of our Kemeny-based strategies are
                   always better and in many cases substantially so.},
  doi =           {10.1109/TAC.2015.2426317},
}

@article{MG-SJ-FB:17b,
  author =        {M. George and S. Jafarpour and F. Bullo},
  journal =       {IEEE Transactions on Automatic Control},
  month =         may,
  note =          {Submitted},
  title =         {Markov Chains with Maximum Entropy for Robotic
                   Surveillance},
  year =          {2017},
  abstract =      {This article provides a comprehensive analysis of the
                   following optimization problem: maximize the entropy
                   rate generated by a Markov chain over a connected
                   graph of order~$n$ and subject to a prescribed
                   stationary distribution. First, we show that this
                   problem is strictly convex with global optimum lying
                   in the interior of the feasible space. Second, using
                   Lagrange multipliers we provide a closed-form
                   expression for the maxentropic Markov chain as a
                   function of an $n$-dimensional vector, referred to as
                   the maxentropic vector; we provide a
                   provably-converging iteration to compute this vector.
                   Third, we show that the maxentropic Markov chain is
                   reversible, compute its entropy rate, and describe
                   special cases, among other results. Fourth, through
                   analysis and simulations, we show that our proposed
                   procedure is more computationally efficient than
                   semidefinite programming methods. Finally, we apply
                   these results to robotic surveillance problems. We
                   show realizations of the maxentropic Markov chains
                   over prototypical robotic roadmaps and find that
                   maxentropic Markov chains outperform minimum mean
                   hitting time Markov chains for so-called
                   ``intelligent intruders'' with short attack
                   durations.},
}

@article{JJH:05,
  author =        {J. J. Hunter},
  journal =       {Linear Algebra and its Applications},
  pages =         {217-243},
  title =         {Stationary distributions and mean first passage times
                   of perturbed {M}arkov chains},
  volume =        {410},
  year =          {2005},
  doi =           {10.1016/j.laa.2005.08.005},
}

@article{BCC-RMJ-VDB:14,
  author =        {B. C. Csáji and R. M. Jungers and V. D. Blondel},
  journal =       {Discrete Applied Mathematics},
  pages =         {73-87},
  title =         {PageRank optimization by edge selection},
  volume =        {169},
  year =          {2014},
  abstract =      {Abstract The importance of a node in a directed graph
                   can be measured by its PageRank. The PageRank of a
                   node is used in a number of application
                   contexts–including ranking websites–and can be
                   interpreted as the average portion of time spent at
                   the node by an infinite random walk. We consider the
                   problem of maximizing the PageRank of a node by
                   selecting some of the edges from a set of edges that
                   are under our control. By applying results from
                   Markov decision theory, we show that an optimal
                   solution to this problem can be found in polynomial
                   time. Our core solution results in a linear
                   programming formulation, but we also provide an
                   alternative greedy algorithm, a variant of policy
                   iteration, which runs in polynomial time, as well.
                   Finally, we show that, under the slight modification
                   for which we are given mutually exclusive pairs of
                   edges, the problem of PageRank optimization becomes
                   NP-hard.},
  doi =           {10.1016/j.dam.2014.01.007},
}

@article{GC-FF:15,
  author =        {G. Como and F. Fagnani},
  journal =       {IEEE Transactions on Network Science and Engineering},
  number =        {2},
  pages =         {53-64},
  title =         {Robustness of Large-Scale Stochastic Matrices to
                   Localized Perturbations},
  volume =        {2},
  year =          {2015},
  doi =           {10.1109/TNSE.2015.2438818},
}

@misc{VA-AKS:17,
  author =        {V. Amelkin and A. K. Singh},
  note =          {arXiv preprint},
  title =         {Disabling External Influence in Social Networks via
                   Edge Recommendation},
  year =          {2017},
  url =           {https://arxiv.org/abs/1709.08139},
}

@article{THS-IS:13,
  author =        {T. H. Summers and I. Shames},
  journal =       {Europhysics Letters},
  number =        {1},
  pages =         {18001},
  title =         {Active influence in dynamical models of structural
                   balance in social networks},
  volume =        {103},
  year =          {2013},
  doi =           {10.1209/0295-5075/103/18001},
}


@article{kahneman1979prospect,
  title={Prospect theory: {A}n analysis of decision under risk},
  author={Kahneman, Daniel and Tversky, Amos},
  journal={Econometrica: Journal of the Econometric Society},
  pages={263-291},
  year={1979},
  publisher={JSTOR}
}

@inproceedings{borowski2014learning,
  title={Learning efficient correlated equilibria},
  author={Borowski, Holly P and Marden, Jason R and Shamma, Jeff S},
  booktitle={53rd Annual Conference on Decision and Control (CDC)},
  pages={6836-6841},
  year={2014},
  organization={IEEE}
}

@inproceedings{marden17selecting,
  title={Selecting efficient correlated equilibria through distributed learning},
  author={Marden, Jason R},
  booktitle={working paper},
  year={2017}
}

@inproceedings{schulmanduality,
  title={The duality gap for two-team zero-sum games},
  author={Schulman, Leonard J and Vazirani, Umesh V},
  booktitle={Innovations in Theoretical Computer Science},
  year={2018}
}


@article{rosen1965existence,
  title={Existence and uniqueness of equilibrium points for concave $n$-person games},
  author={Rosen, J Ben},
  journal={Econometrica: Journal of the Econometric Society},
  pages={520--534},
  year={1965},
  publisher={JSTOR}
}


@article{razaviyayn2013unified,
  title={A unified convergence analysis of block successive minimization methods for nonsmooth optimization},
  author={Razaviyayn, Meisam and Hong, Mingyi and Luo, Zhi-Quan},
  journal={SIAM Journal on Optimization},
  volume={23},
  number={2},
  pages={1126--1153},
  year={2013},
  publisher={SIAM}
}

@article{hartigan1979algorithm,
  title={A K-Means Clustering Algorithm},
  author={Hartigan, J and Wong, M},
  journal={Journal of the Royal Statistical Society. Series C (Applied Statistics)},
  volume={28},
  number={1},
  pages={100--108},
  year={1979}
}


@article{howson1975new,
  title={A new algorithm for the solution of multi-state dynamic programming problems},
  author={Howson, HR and Sancho, NGF},
  journal={Mathematical Programming},
  volume={8},
  number={1},
  pages={104--116},
  year={1975},
  publisher={Springer}
}


@article{hegselmann2002opinion,
  title={Opinion Dynamics and Bounded Confidence Models, Analysis and Simulation},
  author={Hegselmann, Rainer and Krause, Ulrich},
  journal={Journal of Artificial Societies and Social Simulation},
  volume={5},
  number={3},
  pages={1-33},
  year={2002}
}


@article{friedkin1999social,
  title={Social influence networks and opinion change},
  author={Friedkin, Noah E and Johnsen, Eugene C},
  journal={Advances in Group Processes},
  volume={16},
  number={1},
  pages={1-29},
  year={1999}
}


@phdthesis{lorenzt,
	author="Lorenz, J.",
	year="University of Bremen, 2007",
	title="Repeated averaging and bounded-confidence, modeling, analysis and simulation of continuous opinion dynamics",
}

@article{lorenz2010heterogeneous,
  title={Heterogeneous bounds of confidence: Meet, discuss and find consensus!},
  author={Lorenz, Jan},
  journal={Complexity},
  volume={15},
  number={4},
  pages={43--52},
  year={2010},
  publisher={Wiley Online Library}
}

@article{mirtabatabaei2012opinion,
  title={Opinion dynamics in heterogeneous networks: {C}onvergence conjectures and theorems},
  author={Mirtabatabaei, Anahita and Bullo, Francesco},
  journal={SIAM Journal on Control and Optimization},
  volume={50},
  number={5},
  pages={2763--2785},
  year={2012},
  publisher={SIAM}
}

@article{lorenz2010heterogeneous,
  title={Heterogeneous bounds of confidence: {M}eet, discuss and find consensus!},
  author={Lorenz, Jan},
  journal={Complexity},
  volume={15},
  number={4},
  pages={43--52},
  year={2010},
  publisher={Wiley Online Library}
}

@article{julient,
	author="J. M. Hendrickx",
	year="2011",
	title="Graphs and networks for the analysis of autonomous agent systems",
	journal="Ph.D. Thesis, Universite Catholique de Louvain",
}


@book{Bullo,
  title={Distributed control of robotic networks: {A} mathematical approach to motion coordination algorithms},
  author={Bullo, Francesco and Cortes, Jorge and Martinez, Sonia},
  volume={27},
  year={2009},
  publisher={Princeton University Press}
}

@article{proskurnikov2018tutorial,
  title={A tutorial on modeling and analysis of dynamic social networks. {P}art {II}},
  author={Proskurnikov, Anton V and Tempo, Roberto},
  journal={Annual Reviews in Control},
  pages ={166-190},
  volume ={45},
  year={2018},
  publisher={Elsevier}
}


@article{dong2016dynamics,
  title={Dynamics of linguistic opinion formation in bounded confidence model},
  author={Dong, Yucheng and Chen, Xia and Liang, Haiming and Li, Cong-Cong},
  journal={Information Fusion},
  volume={32},
  pages={52--61},
  year={2016},
  publisher={Elsevier}
}

@article{ye2018evolution,
  title={Evolution of social power in social networks with dynamic topology},
  author={Ye, Mengbin Ben and Liu, Ji and Anderson, Brian DO and Yu, Changbin Brad and Basar, Tamer},
  journal={IEEE Transactions on Automatic Control},
  volume={63},
  pages={3793 - 3808},
  year={2018},
  publisher={IEEE}
}

@inproceedings{wai2015identifying,
  title={Identifying trust in social networks with stubborn agents, with application to market decisions},
  author={Wai, Hoi-To and Scaglione, Anna and Leshem, Amir},
  booktitle={53rd Annual Allerton Conference on Communication, Control, and Computing},
  pages={747--754},
  year={2015},
  organization={IEEE}
}


@inproceedings{mohajer2012convergence,
  title={On Convergence Rate of Scalar {H}egselmann-{K}rause Dynamics},
  author={Mohajer, Soheil and Touri, Behrouz},
  booktitle={Proc. American Control Conference (ACC), 2013},
  pages={206--210},
  year={2013},
  organization={IEEE}
}

@inproceedings{nedic2012multi,
  title={Multi-dimensional {H}egselmann-{K}rause dynamics},
  author={Nedi\'c, Angelia and Touri, Behrouz},
  booktitle={Proc. 2012 IEEE 51st Annual Conference on Decision and Control (CDC)},
  pages={68--73},
  year={2012},
  organization={IEEE}
}

@article{behrouzt,
	author="B. Touri",
	year="2011",
	title="Product of Random Stochastic Matrices and Distributed Averaging",
	journal="PhD Thesis, Department of Industrial Engineering, UIUC",
}

@article{degroot1974reaching,
  title={Reaching a consensus},
  author={DeGroot, Morris H},
  journal={Journal of the American Statistical Association},
  volume={69},
  number={345},
  pages={118--121},
  year={1974},
  publisher={Taylor \& Francis}
}

@article{alex,
	author="A. Olshevsky and J. Tsitsiklis",
	year="2008",
	title="On the nonexistence of quadratic {L}yapunov functions
for consensus algorithms",
	journal="IEEE Transactions on Automatic Control",
   volume="53",
	pages="2642--2645"
}


@inproceedings{TouriNedich:CDC2012,
  title={On existence of a quadratic comparison function for random weighted averaging dynamics and its implications},
  author={Touri, Behrouz and Nedi\'c, Angelia},
  booktitle={Proc. 50th IEEE Conference on Decision and Control and European Control Conference (CDC-ECC)},
  pages={3806--3811},
  year={2011},
  organization={IEEE}
}

@article{jadbabaie2003coordination,
  title={Coordination of groups of mobile autonomous agents using nearest neighbor rules},
  author={Jadbabaie, Ali and Lin, Jie and Morse, A Stephen},
  journal={IEEE Transactions on Automatic Control},
  volume={48},
  number={6},
  pages={988--1001},
  year={2003},
  publisher={IEEE}
}

@article{olfati2004consensus,
  title={Consensus problems in networks of agents with switching topology and time-delays},
  author={Olfati-Saber, Reza and Murray, Richard M},
  journal={IEEE Transactions on Automatic Control},
  volume={49},
  number={9},
  pages={1520--1533},
  year={2004},
  publisher={IEEE}
}

@article{zhang2012lyapunov,
  title={Lyapunov, adaptive, and optimal design techniques for cooperative systems on directed communication graphs},
  author={Zhang, Hongwei and Lewis, Frank L and Qu, Zhihua},
  journal={IEEE Transactions on Industrial Electronics},
  volume={59},
  number={7},
  pages={3026--3041},
  year={2012},
  publisher={IEEE}
}

@inproceedings{bhattacharyya2013convergence,
  title={On the convergence of the {H}egselmann-{K}rause system},
  author={Bhattacharyya, Arnab and Braverman, Mark and Chazelle, Bernard and Nguyen, Huy L},
  booktitle={Proceedings of the 4th Conference on Innovations in Theoretical Computer Science},
  pages={61--66},
  year={2013},
  organization={ACM}
}

@inproceedings{roozbehani2008lyapunov,
  title={Lyapunov analysis of quadratically symmetric neighborhood consensus algorithms},
  author={Roozbehani, Mardavij and Megretski, Alexandre and Frazzoli, Emilio},
  booktitle={Proc. 47th IEEE Conference on Decision and Control (CDC)},
  pages={2252--2257},
  year={2008},
  organization={IEEE}
}


@article{hendrickx2013symmetric,
  title={On symmetric continuum opinion dynamics},
  author={Hendrickx, Julien M and Olshevsky, Alex},
  journal={SIAM Journal on Control and Optimization},
  volume={54},
  number={5},
  pages={2893--2918},
  year={2016},
  publisher={SIAM}
}

@inproceedings{blondel20072r,
  title={On the {$2R$} conjecture for multi-agent systems},
  author={Blondel, Vincent D and Hendrickx, Julien M and Tsitsiklis, John N},
  booktitle={European Control Conference (ECC)},
  pages={874--881},
  year={2007},
  organization={IEEE}
}


@article{lorenz2007continuous,
  title={Continuous opinion dynamics under bounded confidence: A survey},
  author={Lorenz, Jan},
  journal={International Journal of Modern Physics C},
  volume={18},
  number={12},
  pages={1819--1838},
  year={2007},
  publisher={World Scientific}
}

@article{chazelle2011total,
  title={The total s-energy of a multiagent system},
  author={Chazelle, Bernard},
  journal={SIAM Journal on Control and Optimization},
  volume={49},
  number={4},
  pages={1680--1706},
  year={2011},
  publisher={SIAM}
}



@article{chazelle2017inertial,
  title={Inertial {H}egselmann-{K}rause systems},
  author={Chazelle, Bernard and Wang, Chu},
  journal={IEEE Transactions on Automatic Control},
  volume={62},
  number={8},
  pages={3905--3913},
  year={2017},
  publisher={IEEE}
}

@article{pineda2013noisy,
  title={The noisy {H}egselmann-{K}rause model for opinion dynamics},
  author={Pineda, Miguel and Toral, Ra{\'u}l and Hern{\'a}ndez-Garc{\'\i}a, Emilio},
  journal={The European Physical Journal B},
  volume={86},
  number={12},
  pages={1--10},
  year={2013},
  publisher={Springer}
}

@article{etesami2018influence,
  title={Influence of conformist and manipulative behaviors on public opinion},
  author={Etesami, S Rasoul and Bolouki, Sadegh and Nedich, Angelia and Basar, Tamer and Poor, H Vincent},
  journal={IEEE Transactions on Control of Network Systems},
  year={2018},
  publisher={IEEE}
}

@article{el2017managing,
  title={Managing price uncertainty in prosumer-centric energy trading: A prospect-theoretic Stackelberg game approach},
  author={El Rahi, Georges and Etesami, S Rasoul and Saad, Walid and Mandayam, Narayan and Poor, H Vincent},
  journal={IEEE Transactions on Smart Grid},
  year={2017},
  publisher={IEEE}
}

@article{etesami2018stochastic,
  title={Stochastic Games for Smart Grid Energy Management with Prospect Prosumers},
  author={Etesami, S Rasoul and Saad, Walid and Mandayam, Narayan and Poor, H Vincent},
  journal={IEEE Transactions on Automatic Control},
  year={2018},
  publisher={IEEE}
}

@article{truong2018optimal,
  title={Optimal Attack Strategies Against Predictors-Learning From Expert Advice},
  author={Truong, Anh and Etesami, S Rasoul and Etesami, Jalal and Kiyavash, Negar},
  journal={IEEE Transactions on Information Forensics and Security},
  volume={13},
  number={1},
  pages={6--19},
  year={2018},
  publisher={IEEE}
}

@article{etesami2017price,
  title={Price of anarchy and an approximation algorithm for the binary-preference capacitated selfish replication game},
  author={Etesami, Seyed Rasoul and Ba{\c{s}}ar, Tamer},
  journal={Automatica},
  volume={76},
  pages={153--163},
  year={2017},
  publisher={Elsevier}
}

@article{etesami2016pure,
  title={Pure {N}ash equilibrium in a capacitated selfish resource allocation game},
  author={Etesami, Seyed Rasoul and Basar, Tamer},
  journal={IEEE Transactions on Control of Network Systems},
  year={2016},
  publisher={IEEE}
}

@inproceedings{etesami2017smart,
  title={Smart routing in smart grids},
  author={Etesami, S Rasoul and Saad, Walid and Mandayam, Narayan and Poor, H Vincent},
  booktitle={56th Annual Conference on Decision and Control (CDC)},
  pages={2599--2604},
  year={2017},
  organization={IEEE}
}

@book{etesami2017potential,
  title={Potential-based analysis of social, communication, and distributed networks},
  author={Etesami, S. Rasoul},
  year={2017},
  publisher={Springer}
}

@inproceedings{etesami2013termination,
  title={Termination time of multidimensional {H}egselmann-{K}rause opinion dynamics},
  author={Etesami, Seyed Rasoul and Ba{\c{s}}ar, Tamer and Nedi{\'c}, Angelia and Touri, Behrouz},
  booktitle={American Control Conference (ACC)},
  pages={1255--1260},
  year={2013},
  organization={IEEE}
}

@article{olshevsky2009convergence,
  title={Convergence speed in distributed consensus and averaging},
  author={Olshevsky, Alex and Tsitsiklis, John N},
  journal={SIAM Journal on Control and Optimization},
  volume={48},
  number={1},
  pages={33--55},
  year={2009},
  publisher={SIAM}
}

@article{nedic2009distributed,
  title={On distributed averaging algorithms and quantization effects},
  author={Nedic, Angelia and Olshevsky, Alex and Ozdaglar, Asuman and Tsitsiklis, John N},
  journal={IEEE Transactions on Automatic Control},
  volume={54},
  number={11},
  pages={2506--2517},
  year={2009},
  publisher={IEEE}
}

@article{nedic2015distributed,
  title={Distributed optimization over time-varying directed graphs},
  author={Nedi{\'c}, Angelia and Olshevsky, Alex},
  journal={IEEE Transactions on Automatic Control},
  volume={60},
  number={3},
  pages={601--615},
  year={2015},
  publisher={IEEE}
}

@article{bacsar2016convergence,
  title={Convergence time of quantized {M}etropolis consensus over time-varying networks},
  author={Ba{\c{s}}ar, Tamer and Etesami, Seyed Rasoul and Olshevsky, Alex},
  journal={IEEE Transactions on Automatic Control},
  volume={61},
  number={12},
  pages={4048--4054},
  year={2016},
  publisher={IEEE}
}

@article{zhu2011convergence,
  title={On the convergence time of asynchronous distributed quantized averaging algorithms},
  author={Zhu, Minghui and Mart{\'\i}nez, Sonia},
  journal={IEEE Transactions on Automatic Control},
  volume={56},
  number={2},
  pages={386--390},
  year={2011},
  publisher={IEEE}
}

@article{tatarenko2017non,
  title={Non-convex distributed optimization},
  author={Tatarenko, Tatiana and Touri, Behrouz},
  journal={IEEE Transactions on Automatic Control},
  volume={62},
  number={8},
  pages={3744--3757},
  year={2017},
  publisher={IEEE}
}

@article{olfati2004consensus,
  title={Consensus problems in networks of agents with switching topology and time-delays},
  author={Olfati-Saber, Reza and Murray, Richard M},
  journal={IEEE Transactions on automatic control},
  volume={49},
  number={9},
  pages={1520--1533},
  year={2004},
  publisher={IEEE}
}

@article{hendrickx2013convergence,
  title={Convergence of type-symmetric and cut-balanced consensus seeking systems},
  author={Hendrickx, Julien M and Tsitsiklis, John N},
  journal={IEEE Transactions on Automatic Control},
  volume={58},
  number={1},
  pages={214--218},
  year={2013},
  publisher={IEEE}
}

@article{jadbabaie2003coordination,
  title={Coordination of groups of mobile autonomous agents using nearest neighbor rules},
  author={Jadbabaie, Ali and Lin, Jie and Morse, A Stephen},
  journal={IEEE Transactions on automatic control},
  volume={48},
  number={6},
  pages={988--1001},
  year={2003},
  publisher={IEEE}
}

@article{degroot1974reaching,
  title={Reaching a consensus},
  author={DeGroot, Morris H},
  journal={Journal of the American Statistical Association},
  volume={69},
  number={345},
  pages={118--121},
  year={1974},
  publisher={Taylor \& Francis Group}
}

@article{friedkin1997social,
  title={Social positions in influence networks},
  author={Friedkin, Noah E and Johnsen, Eugene C},
  journal={Social Networks},
  volume={19},
  number={3},
  pages={209--222},
  year={1997},
  publisher={Elsevier}
}

@article{nedic2018network,
  title={Network topology and communication-computation tradeoffs in decentralized optimization},
  author={Nedi{\'c}, Angelia and Olshevsky, Alex and Rabbat, Michael G},
  journal={Proceedings of the IEEE},
  volume={106},
  number={5},
  pages={953--976},
  year={2018},
  publisher={IEEE}
}

@book{touri2012product,
  title={Product of random stochastic matrices and distributed averaging},
  author={Touri, Behrouz},
  year={2012},
  publisher={Springer Science \& Business Media}
}

@inproceedings{touri2011existence,
  title={On existence of a quadratic comparison function for random weighted averaging dynamics and its implications},
  author={Touri, Behrouz and Nedi{\'c}, Angelia},
  booktitle={50th IEEE Conference on Decision and Control and European Control Conference (CDC-ECC)},
  pages={3806--3811},
  year={2011},
  organization={IEEE}
}

@incollection{sonin2008decomposition,
  title={The decomposition-separation theorem for finite nonhomogeneous {M}arkov chains and related problems},
  author={Sonin, Isaac M and others},
  booktitle={Markov Processes and Related Topics: A Festschrift for Thomas G. Kurtz},
  pages={1--15},
  year={2008},
  publisher={Institute of Mathematical Statistics}
}

@inproceedings{etesami2013termination,
  title={Termination time of multidimensional {H}egselmann-{K}rause opinion dynamics},
  author={Etesami, Seyed Rasoul and Ba{\c{s}}ar, Tamer and Nedi{\'c}, Angelia and Touri, Behrouz},
  booktitle={American Control Conference (ACC)},
  pages={1255--1260},
  year={2013},
  organization={IEEE}
}


@article{su2017partial,
  title={Partial convergence of heterogeneous {H}egselmann-{K}rause opinion dynamics},
  author={Su, Wei and Gu, YaJuan and Wang, Sha and Yu, YongGuang},
  journal={Science China Technological Sciences},
  volume={60},
  number={9},
  pages={1433--1438},
  year={2017},
  publisher={Springer}
}

@article{monderer1996potential,
  title={Potential games},
  author={Monderer, Dov and Shapley, Lloyd S},
  journal={Games and Economic Behavior},
  volume={14},
  number={1},
  pages={124--143},
  year={1996},
  publisher={Elsevier}
}

@article{attouch2010proximal,
  title={Proximal alternating minimization and projection methods for nonconvex problems: {A}n approach based on the Kurdyka-{\L}ojasiewicz inequality},
  author={Attouch, H{\'e}dy and Bolte, J{\'e}r{\^o}me and Redont, Patrick and Soubeyran, Antoine},
  journal={Mathematics of Operations Research},
  volume={35},
  number={2},
  pages={438--457},
  year={2010},
  publisher={INFORMS}
}


@inproceedings{etesami2019sequential,
  title={Sequential Optimization for State-Dependent Opinion Dynamics},
  author={Etesami, S. Rasoul},
  booktitle={American Control Conference (ACC), Philadelphia, PA, USA, July 10-12},
  year={2019},
  organization={IEEE}
}

@article{etesami2016convergence,
  title={Convergence time for unbiased quantized consensus over static and dynamic networks},
  author={Etesami, Seyed Rasoul and Ba{\c{s}}ar, Tamer},
  journal={IEEE Transactions on Automatic Control},
  volume={61},
  number={2},
  pages={443--455},
  year={2016},
  publisher={IEEE}
}

@book{etesami2017potential,
  title={Potential-based analysis of social, communication, and distributed networks},
  author={Etesami, Seyed Rasoul},
  year={2017},
  publisher={Springer}
}

@article{etesami2019simple,
  title={A Simple Framework for Stability Analysis of State-Dependent Networks of Heterogeneous Agents},
  author={Etesami, S Rasoul},
  journal={SIAM Journal on Control and Optimization},
  volume={57},
  number={3},
  pages={1757--1782},
  year={2019},
  publisher={SIAM}
}

@article{etesami2019dynamic,
  title={Dynamic Games in Cyber-Physical Security: An Overview},
  author={Etesami, S Rasoul and Ba{\c{s}}ar, Tamer},
  journal={Dynamic Games and Applications},
  pages={1--30},
  publisher={Springer}
}

@book{bullo2009distributed,
  title={Distributed {C}ontrol of {R}obotic {N}etworks: {A} {M}athematical {A}pproach to {M}otion {C}oordination {A}lgorithms},
  author={Bullo, Francesco and Cortes, Jorge and Martinez, Sonia},
  volume={27},
  year={2009},
  publisher={Princeton University Press}
}

@inproceedings{blondel2005convergence,
  title={Convergence in multiagent coordination, consensus, and flocking},
  author={Blondel, Vincent D and Hendrickx, Julien M and Olshevsky, Alex and Tsitsiklis, John N},
  booktitle={Proceedings of the 44th IEEE Conference on Decision and Control},
  pages={2996--3000},
  year={2005},
  organization={IEEE}
}

@book{levin2017markov,
  title={Markov {C}hains and {M}ixing {T}imes},
  author={Levin, David A and Peres, Yuval},
  volume={107},
  year={2017},
  publisher={American Mathematical Soc.}
}

@article{burger2012hierarchical,
  title={Hierarchical clustering of dynamical networks using a saddle-point analysis},
  author={Burger, Mathias and Zelazo, Daniel and Allgower, Frank},
  journal={IEEE Transactions on Automatic Control},
  volume={58},
  number={1},
  pages={113--124},
  year={2012},
  publisher={IEEE}
}

@article{burger2014duality,
  title={Duality and network theory in passivity-based cooperative control},
  author={B{\"u}rger, Mathias and Zelazo, Daniel and Allg{\"o}wer, Frank},
  journal={Automatica},
  volume={50},
  number={8},
  pages={2051--2061},
  year={2014},
  publisher={Elsevier}
}

@article{proskurnikov2018tutorial,
  title={A tutorial on modeling and analysis of dynamic social networks. {P}art {II}},
  author={Proskurnikov, Anton V and Tempo, Roberto},
  journal={Annual Reviews in Control},
  pages ={166-190},
  volume ={45},
  year={2018},
  publisher={Elsevier}
}

@book{arrow1958studies,
  title={Studies in {L}inear and {N}on-linear {P}rogramming},
  author={Arrow, Kenneth J and Hurwicz, Leonid and Uzawa, Hirofumi},
  year={1958},
  publisher={Cambridge University Press}
}

@article{feijer2010stability,
  title={Stability of primal-dual gradient dynamics and applications to network optimization},
  author={Feijer, Diego and Paganini, Fernando},
  journal={Automatica},
  volume={46},
  number={12},
  pages={1974--1981},
  year={2010},
  publisher={Elsevier}
}

@article{bubeck2015convex,
  title={Convex optimization: {A}lgorithms and complexity},
  author={Bubeck, S{\'e}bastien and others},
  journal={Foundations and Trends{\textregistered} in Machine Learning},
  volume={8},
  number={3-4},
  pages={231--357},
  year={2015},
  publisher={Now Publishers, Inc.}
}

@article{jabin2014clustering,
  title={Clustering and asymptotic behavior in opinion formation},
  author={Jabin, Pierre-Emmanuel and Motsch, Sebastien},
  journal={Journal of Differential Equations},
  volume={257},
  number={11},
  pages={4165--4187},
  year={2014},
  publisher={Elsevier}
}

@book{boyd2004convex,
  title={Convex {O}ptimization},
  author={Boyd, Stephen and Vandenberghe, Lieven},
  year={2004},
  publisher={Cambridge University Press}
}
